R4Dyn: Exploring Radar for Self-Supervised Monocular Depth Estimation of Dynamic Scenes

While self-supervised monocular depth estimation in driving scenarios has achieved comparable performance to supervised approaches, violations of the static world assumption can still lead to erroneous depth predictions of traffic participants, posing a potential safety issue. In this paper, we present R4Dyn, a novel set of techniques to use cost-efficient radar data on top of a self-supervised depth estimation framework. In particular, we show how radar can be used during training as weak supervision signal, as well as an extra input to enhance the estimation robustness at inference time. Since automotive radars are readily available, this allows to collect training data from a variety of existing vehicles. Moreover, by filtering and expanding the signal to make it compatible with learning-based approaches, we address radar inherent issues, such as noise and sparsity. With R4Dyn we are able to overcome a major limitation of self-supervised depth estimation, i.e. the prediction of traffic participants. We substantially improve the estimation on dynamic objects, such as cars by 37% on the challenging nuScenes dataset, hence demonstrating that radar is a valuable additional sensor for monocular depth estimation in autonomous vehicles.

==> tables/architectures.tex <==
% \begin{table*}
% \begin{center}
% \begin{tabular}{c|l|c|c|c|cccccccc}
% \toprule
% Arch. & Sup. & In. & \# Ps & AbsRel & SqRel & RMSE & RMSE$_{log}$ & $\delta_1$ & $\delta_2$ & $\delta_3$ \\
% \midrule\midrule
% RN-18 & M+v  & I & 14.8M & 0.131 & 1.705 & 6.520 & 0.229 & 0.857 & 0.944 & 0.972 \\
% RN-18 & M+v+r & I & 14.8M &&&&&&&&\\
% RN-50 & M+v+r & I & 34.6M &&&&&&&&\\
% RN-18 & M+v+r & I+R & 15.9M &&&&&&&&\\
% RN-50 & M+v+r & I+R & 39.7M &&&&&&&&\\
% \bottomrule
% \end{tabular}
% \end{center}
% \caption{Ablation study on the network architecture (Arch.), evaluated on the nuScenes~\cite{2020-caesar} validation set excluding night and rain scenes. RN-18 and RN-50 denote ResNet~\cite{2016-kaiming} backbones with 18 and 50 layers respectively. All methods are pretrained on ImageNet~\cite{2009-deng}. \# Ps refers to the number of model parameters of the depth network only.}
% \label{table:architecture}
% \end{table*}

\begin{table}
\begin{center}
\begin{tabular}{l|ccc|cc}
\toprule
Arch. & Sup. & In. & M.P. & AbsRel & AbsRel$_\text{C}$\\
\midrule\midrule
RN18 & M+v  & Im & 14.8 & 0.1315 & 0.1862 \\  %vehicle:0.2091
RN18 & M+v+r & Im & 14.8 & 0.1296 & 0.1343 \\
RN18 & M+v+r & ImR & 15.9 & 0.1259 & 0.1250 \\%vehicle:0.1504
RN50 & M+v & Im & 34.6 & 0.1301 & 0.1779 \\ % vehicle: 0.2047
RN50 & M+v+r & Im & 34.6 &  & \\
RN50 & M+v+r & ImR & 39.7 &. & \\
\bottomrule
\end{tabular}
\end{center}
\caption{Comparison of network architectures (Arch.) on the nuScenes~\cite{2020-caesar} validation \textit{day-clear} set. RN18 and RN50 are ResNet~\cite{2016-kaiming} backbones with different sizes. M.P. refers to the millions of model parameters of the depth network.}
\label{table:network_architectures}
\end{table}
